Scenario-Based Test Reduction and Prioritization for Multi-Module Autonomous Driving Systems

When developing autonomous driving systems (ADS), developers often need to replay previously collected driving recordings to check the correctness of newly introduced changes to the system. However, simply replaying the entire recording is not necessary given the high redundancy of driving scenes in a recording (e.g., keeping the same lane for 10 minutes on a highway). In this paper, we propose a novel test reduction and prioritization approach for multi-module ADS. First, our approach automatically encodes frames in a driving recording to feature vectors based on a driving scene schema. Then, the given recording is sliced into segments based on the similarity of consecutive vectors. Lengthy segments are truncated to reduce the length of a recording and redundant segments with the same vector are removed. The remaining segments are prioritized based on both the coverage and the rarity of driving scenes. We implemented this approach on an industry level, multi-module ADS called Apollo and evaluated it on three road maps in various regression settings. The results show that our approach significantly reduced the original recordings by over 34% while keeping comparable test effectiveness, identifying almost all injected faults. Furthermore, our test prioritization method achieves about 22% to 39% and 41% to 53% improvements over three baselines in terms of both the average percentage of faults detected (APFD) and TOP-K.

==> intro_backup.tex <==
\section{Introduction}

Autonomous driving has developed rapidly in recent years. Many companies such as Google Waymo and Baidu have launched Robotaxi services powered by autonomous driving systems (ADSs).  However, the safety of autonomous driving is still a concern in public due to traffic accidents involving autonomous vehicles~\cite{tesla, waymo_accident, petrovic2020traffic}. To improve the safety of autonomous vehicles, autonomous vehicle companies often apply long-distance on-road testing and simulation testing. The first aim is to evaluate the performance of ADSs under diverse and rare driving scenarios. In addition, during the testing, large amounts of driving recordings are collected for further improvement and regression testing of ADSs.   

A driving recording contains rich information such as environmental images and other sensor data. These driving recordings are useful for making testing cases. However, currently there are some problems on the use of collected driving recordings. First, the process of driving recordings requires huge human effort. Testers need to manually classify, label, and then select driving scenarios from the driving data. Second, the test effectiveness on collected driving data is low. Redundant and similar driving scenarios are used to test ADSs, which is not helpful for comprehensively finding potential problems in ADSs. In addition, how to detect problems in ADSs as soon as possible given long driving recordings is a question. Third, current main-stream multi-module ADSs cannot be thoroughly tested using collected driving recordings. As shown in Figure~\ref{fig:ads}, an industrial-level ADS contains multiple modules. The perception module processes sensor inputs such as images and point clouds to detect obstacles and traffic lights in the driving scene using different Convolutional Neural Networks (CNNs)~\cite{yamashita2018convolutional}. The prediction module estimates trajectories of detected obstacles. The planning module generates the trajectory of the autonomous vehicle (often called ego-vehicle) based on outputs of perception and prediction modules. The control module finally outputs the control commands such as steering angle and accelerations. 
All modules should be tested intensively using collected driving recordings. However, currently driving recordings are often used to evaluate the final output of ADSs (e.g., collision or deviation)~\cite{tang2021systematic}. They are not used to evaluate performances of ADSs in module level. For example, from a driving recording we can extract a red light scenario to evaluate the traffic light detection system in the perception module and a overtake scenario to evaluate the planning module. 

Even though some works are proposed for ADS testing, most of them~\cite{zhang2018deeproad, tian2018deeptest, zhou2020deepbillboard, gambi2019generating} focus on test case generation and their test targets are Eend-to-End (E2E) driving models. a few work start exploring test selection and prioritization for ADS.~\cite{birchler2021automated} works on a lane keeping system and the system under test (SUT) is also E2E driving models. The definition of scenarios in the paper are maps with different road conditions, which are different from driving scenarios in most work. Therefore, to solve above problems and fill the research gap, we propose scenario-based testing reduction and prioritization methods for regression testing on ADS modules. We observe that for ADSs with Robot Operating System (ROS) or similar subscribe-publish communication system, collected driving recordings contain not only driving environment information but also module outputs of ADSs. Leveraging these outputs, we design and extract feature vectors to represent rich semantic information for each frame in a driving recording. Then, the recording is split into multiple driving segments according to the difference of frame features. Each segment is corresponding to a driving scenario and represented by a segment feature vector. To reduce the test time, for each segment we only keep part of it to drop redundant driving scenes (e.g., go straight for long time on the highway). We also drop similar driving segments that have the same segment feature vector to remove duplicated driving scenarios.
Furthermore, we analyze the rarity of kept driving segments and sort them from rare to common driving scenarios. The prioritized driving segments further improve the efficiency of finding potential problems in an ADS module.        


% Now industrial companies normally adopt multi-module architecture ADSs because they are easier to debug and test. A multi-module ADS normally contains perception, prediction, planning and control modules. Each module contains many neural networks or code blocks to deal with different tasks. Specifically, the perception module processes sensor inputs such as images and point clouds to detect obstacles and traffic lights in the driving scene using different Convolutional Neural Networks (CNNs). The prediction module estimates trajectories of detected obstacles. The planning module generates the trajectory of the autonomous vehicle (often called ego-vehicle) based on outputs of perception and prediction modules. The control module finally outputs the control commands such as steering angle and accelerations. These modules run in subscribe-publish mechanism based on Robot Operating System (ROS) or similar framework such as CyberRT. 

% When an autonomous vehicle is running on road or in simulation, a driving recording file is saved, which contains the sensor inputs of the driving environment as well as outputs of all modules. The driving recording is further used for regression testing once a module is updated. For example, when the perception module is updated, it is tested on the sensor input data in the driving recording to ensure no new bugs are introduced after the update. Unlike testing traditional software that deterministic test data can be synthesis when needed, the on-road test data can only be recorded during the test. Therefore, the reuse of driving recording for regression testing is a crucial way to make the use of driving data and test ADSs. However, test efficiency is a problem in the regression testing based on the driving recording. First, the recording normally contains many repeated driving scenarios such as traveling along a highway. Testing on such repeated scenarios costs large amount of time while detects few bugs. In addition, in an update of a module, a few code blocks or neural networks are modified. The modified code or neural network is normally only related to certain driving scenarios in the driving recording. In this condition, applying regression testing on the entire driving recording is a waste of time.    

% Now how to speed up the testing of autonomous driving systems is an urgent problem to solve. 

  

To evaluate our method, we conduct experiments in a simulator LGSVL~\cite{rong2020lgsvl} on an industrial multi-module ADS Baidu Apollo~\cite{Apollo}. We first collect driving recordings on three maps in LGSVL as the driving recording benchmark. Then we inject mutants into the source code of modules to simulate the update of modules while introducing potential new bugs. Specifically, we create a regression benchmark containing nine modified perception modules (traffic light detection and obstacle detection sub-modules), prediction modules, and planning modules respectively. For each driving recording benchmark, we first split it into recording segments and then apply test reduction and prioritization on segments. We finally evaluate 1) to what extent the overall testing time reduces; 2) whether driving segments after reduction have the same ability to detect potential problems in an ADS as original driving segments; 3) whether driving segments after prioritization find potential module problems faster compared with two baselines. The experiment results show that the test reduction method helps to decrease over 50\% testing time. The selected recording segments keep the similar capability to detect over 99.7\% potential problems in ADS modules as the original driving recording. The test prioritization method improve the test efficiency at most  190\%.  

There are three main contributions of this work:
\begin{itemize}
    \item We propose a scenario-based test reduction and prioritization method for regression testing on multi-module ADSs. 
    
    \item We create a regression testing benchmark including driving recordings on three maps and 10 modified perception modules (traffic light detection and obstacle detection sub-modules), prediction modules, and planning modules.
    
    \item We conduct experiments on the industry-level ADS Baidu Apollo. The experiment results show the effectiveness of the proposed method.
\end{itemize}


==> result_backup.tex <==
\section{Evaluation}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{comment}
\begin{table*}
\centering
\caption{Test prioritization on perception module}
\begin{tabular}{c|l|llllll} 
\hline
\multirow{7}{*}{\textbf{Bug 1}} & \multirow{2}{*}{}                                & \multicolumn{2}{l|}{Baseline\_order}                                                                  & \multicolumn{2}{l|}{Baseline\_random}                                                                & \multicolumn{2}{l}{Proposed method}                                                                    \\ 
\cline{3-8}
                                &                                                  & Top K                                           & AFPD                                                & Top K                                            & AFPD                                              & Top K                                           & AFPD                                                 \\ 
\cline{2-8}
                                & Test Suite 1\textbf{ }                           & \textbf{1 }                                     & \textbf{0.938 }                                     & 1.2                                              & 0.9125                                            & \textbf{1 }                                     & \textbf{0.938 }                                      \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1 } & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.875}  & {\cellcolor[rgb]{0.937,0.937,0.937}}2.2          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.575         & {\cellcolor[rgb]{0.937,0.937,0.937}}2           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.625            \\
                                & Test Suite 3\textbf{ }                           & 2                                               & 0.750                                               & \textbf{1.7}                                     & \textbf{0.8}                                      & 2                                               & \textbf{0.750 }                                      \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1 } & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.833 } & {\cellcolor[rgb]{0.937,0.937,0.937}}2.9          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.6           & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1 } & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.833 }  \\
                                & Test Suite 5                                     & \textbf{1 }                                     & \textbf{0.833 }                                     & 1.5                                              & 0.67                                              & \textbf{1 }                                     & \textbf{0.833 }                                      \\ 
\hline
\multirow{5}{*}{\textbf{Bug 2}} & Test Suite 1                                     & \textbf{1 }                                     & \textbf{0.938 }                                     & 2.2                                              & 0.7875                                            & \textbf{1 }                                     & \textbf{0.938 }                                      \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}3           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.375           & {\cellcolor[rgb]{0.937,0.937,0.937}}2.2          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.575         & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.875 }  \\
                                & Test Suite 3                                     & -1                                              & -1                                                  & -1                                               & -1                                                & -1                                              & -1                                                   \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1              & {\cellcolor[rgb]{0.937,0.937,0.937}}-1           & {\cellcolor[rgb]{0.937,0.937,0.937}}-1            & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1               \\
                                & Test Suite 5                                     & -1                                              & -1                                                  & -1                                               & -1                                                & -1                                              & -1                                                   \\ 
\hline
\multirow{5}{*}{\textbf{Bug 3}} & Test Suite 1                                     & \textbf{1 }                                     & \textbf{0.938 }                                     & 1.9                                              & 0.825                                             & \textbf{1 }                                     & \textbf{0.938 }                                      \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1 } & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.875 } & {\cellcolor[rgb]{0.937,0.937,0.937}}2            & {\cellcolor[rgb]{0.937,0.937,0.937}}0.625         & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.875 }  \\
                                & Test Suite 3\textbf{ }                           & 3                                               & 0.583                                               & 1.2                                              & 0.89                                              & \textbf{1}                                      & \textbf{0.917}                                       \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}4           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.417           & {\cellcolor[rgb]{0.937,0.937,0.937}}2.1          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.73          & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.917}   \\
                                & Test Suite 5                                     & \textbf{1}                                      & \textbf{0.833}                                      & 1.4                                              & 0.7                                               & \textbf{1}                                      & \textbf{0.833}                                       \\ 
\hline
\multirow{5}{*}{\textbf{Bug 4}} & Test Suite 1                                     & \textbf{2}                                      & \textbf{0.85}                                       & 3.6                                              & 0.69                                              & 4                                               & 0.65                                                 \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1              & {\cellcolor[rgb]{0.937,0.937,0.937}}-1           & {\cellcolor[rgb]{0.937,0.937,0.937}}-1            & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1               \\
                                & Test Suite 3                                     & -1                                              & -1                                                  & -1                                               & -1                                                & -1                                              & -1                                                   \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{3}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.69}   & {\cellcolor[rgb]{0.937,0.937,0.937}}5.6          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.36          & {\cellcolor[rgb]{0.937,0.937,0.937}}7           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.19             \\
                                & Test Suite 5                                     & -1                                              & -1                                                  & -1                                               & -1                                                & -1                                              & -1                                                   \\ 
\hline
\multirow{5}{*}{\textbf{Bug 5}} & Test Suite 1                                     & \textbf{1 }                                     & \textbf{0.95}                                       & \textbf{1}                                       & \textbf{0.95}                                     & \textbf{1 }                                     & \textbf{0.95}                                        \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1 } & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.83}   & {\cellcolor[rgb]{0.937,0.937,0.937}}1.3          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.73          & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.83}    \\
                                & Test Suite 3                                     & \textbf{1}                                      & \textbf{0.9}                                        & 1.2                                              & 0.86                                              & \textbf{1}                                      & \textbf{0.9}                                         \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.94}   & {\cellcolor[rgb]{0.937,0.937,0.937}}1.1          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.93          & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.94}    \\
                                & Test Suite 5                                     & \textbf{1}                                      & \textbf{0.83}                                       & 1.3                                              & 0.73                                              & 2                                               & 0.5                                                  \\ 
\hline
\multirow{5}{*}{\textbf{Bug 6}} & Test Suite 1                                     & \textbf{1 }                                     & \textbf{0.95}                                       & 1.5                                              & 0.90                                              & \textbf{1 }                                     & \textbf{0.95}                                        \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1              & {\cellcolor[rgb]{0.937,0.937,0.937}}-1           & {\cellcolor[rgb]{0.937,0.937,0.937}}-1            & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1               \\
                                & Test Suite 3                                     & -1                                              & -1                                                  & -1                                               & -1                                                & -1                                              & -1                                                   \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1              & {\cellcolor[rgb]{0.937,0.937,0.937}}-1           & {\cellcolor[rgb]{0.937,0.937,0.937}}-1            & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1               \\
                                & Test Suite 5                                     & 3                                               & 0.167                                               & \textbf{1.6}                                     & \textbf{0.63}                                     & 2                                               & 0.5                                                  \\ 
\hline
\multirow{5}{*}{\textbf{Bug 7}} & Test Suite 1                                     & \textbf{3}                                      & \textbf{0.75}                                       & 4.2                                              & 0.63                                              & \textbf{3}                                      & \textbf{0.75}                                        \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1              & {\cellcolor[rgb]{0.937,0.937,0.937}}-1           & {\cellcolor[rgb]{0.937,0.937,0.937}}-1            & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1               \\
                                & Test Suite 3                                     & -1                                              & -1                                                  & -1                                               & -1                                                & -1                                              & -1                                                   \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1              & {\cellcolor[rgb]{0.937,0.937,0.937}}-1           & {\cellcolor[rgb]{0.937,0.937,0.937}}-1            & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1               \\
                                & Test Suite 5                                     & -1                                              & -1                                                  & -1                                               & -1                                                & -1                                              & -1                                                   \\ 
\hline
\multirow{5}{*}{\textbf{Bug 8}} & Test Suite 1                                     & \textbf{1}                                      & \textbf{0.95}                                       & \textbf{1}                                       & \textbf{0.95}                                     & \textbf{1 }                                     & \textbf{0.95}                                        \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}2           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.5             & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1.7} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.6}  & {\cellcolor[rgb]{0.937,0.937,0.937}}2           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.5              \\
                                & Test Suite 3                                     & 2                                               & 0.7                                                 & \textbf{1.9}                                     & \textbf{0.72}                                     & 2                                               & 0.7                                                  \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}3           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.69            & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1.2} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.91} & {\cellcolor[rgb]{0.937,0.937,0.937}}2           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.81             \\
                                & Test Suite 5                                     & \textbf{1 }                                     & \textbf{0.83}                                       & \textbf{1}                                       & \textbf{0.83}                                     & \textbf{1}                                      & \textbf{0.83}                                        \\ 
\hline
\multirow{5}{*}{\textbf{Bug 9}} & Test Suite 1                                     & 9                                               & 0.15                                                & \textbf{6.3}                                     & \textbf{0.42}                                     & 9                                               & 0.15                                                 \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1              & {\cellcolor[rgb]{0.937,0.937,0.937}}-1           & {\cellcolor[rgb]{0.937,0.937,0.937}}-1            & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1               \\
                                & Test Suite 3                                     & -1                                              & -1                                                  & -1                                               & -1                                                & -1                                              & -1                                                   \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1              & {\cellcolor[rgb]{0.937,0.937,0.937}}-1           & {\cellcolor[rgb]{0.937,0.937,0.937}}-1            & {\cellcolor[rgb]{0.937,0.937,0.937}}-1          & {\cellcolor[rgb]{0.937,0.937,0.937}}-1               \\
                                & Test Suite 5                                     & -1                                              & -1                                                  & -1                                               & -1                                                & -1                                              & -1                                                   \\
\hline
\end{tabular}
\end{table*}
\end{comment}

% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table*}
\centering
\caption{Test prioritization on planning module}
\begin{tabular}{c|l|llllll} 
\hline
\multirow{7}{*}{\textbf{Bug 10}} & \multirow{2}{*}{}                                & \multicolumn{2}{l|}{Baseline\_order}                                                                & \multicolumn{2}{l|}{Baseline\_random}                                                                  & \multicolumn{2}{l}{Proposed method}                                                                  \\ 
\cline{3-8}
                                 &                                                  & Top K                                           & AFPD                                              & Top K                                             & AFPD                                               & Top K                                           & AFPD                                               \\ 
\cline{2-8}
                                 & Test Suite 1\textbf{ }                           & \textbf{1 }                                     & \textbf{0.92}                                     & 1.8                                               & 0.78                                               & \textbf{1 }                                     & \textbf{0.92}                                      \\
                                 & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}2           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.83          & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1.0}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{ 0.94} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.94}  \\
                                 & Test Suite 3\textbf{ }                           & 2                                               & 0.79                                              & 1.4                                               & 0.87                                               & \textbf{1}                                      & \textbf{0.93}                                      \\
                                 & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1 } & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.94} & {\cellcolor[rgb]{0.937,0.937,0.937}}1.7           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.87           & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1 } & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.94}  \\
                                 & Test Suite 5                                     & \textbf{1 }                                     & \textbf{0.9}                                      & 1.5                                               & 0.8                                                & 4                                               & 0.3                                                \\ 
\hline
\multirow{5}{*}{\textbf{Bug 11}} & Test Suite 1                                     & \textbf{1 }                                     & \textbf{0.92}                                     & 1.4                                               & 0.85                                               & \textbf{1 }                                     & \textbf{0.92}                                      \\
                                 & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}2           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.83          & {\cellcolor[rgb]{0.937,0.937,0.937}}1.1           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.93           & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.94}  \\
                                 & Test Suite 3                                     & 2                                               & 0.79                                              & 1.75                                              & 0.82                                               & \textbf{1}                                      & \textbf{0.93}                                      \\
                                 & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}4           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.61          & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1.95} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.84}  & {\cellcolor[rgb]{0.937,0.937,0.937}}4           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.61           \\
                                 & Test Suite 5                                     & \textbf{1}                                      & \textbf{0.9}                                      & 1.75                                              & 0.75                                               & 4                                               & 0.3                                                \\ 
\hline
\multirow{5}{*}{\textbf{Bug 12}} & Test Suite 1                                     & \textbf{1 }                                     & \textbf{0.92}                                     & 1.3                                               & 0.87                                               & \textbf{1 }                                     & \textbf{0.92}                                      \\
                                 & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}2           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.83          & {\cellcolor[rgb]{0.937,0.937,0.937}}1.17          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.93           & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.93}  \\
                                 & Test Suite 3\textbf{ }                           & 2                                               & 0.83                                              & 1.9                                               & 0.8                                                & \textbf{1}                                      & \textbf{0.93}                                      \\
                                 & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}4           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.79          & {\cellcolor[rgb]{0.937,0.937,0.937}}2.0           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.83           & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.93}  \\
                                 & Test Suite 5                                     & 4                                               & 0.61                                              & \textbf{2.03}                                     & \textbf{0.69}                                      & 4                                               & 0.61                                               \\ 
\hline
\multirow{5}{*}{\textbf{Bug 13}} & Test Suite 1                                     & \textbf{1}                                      & \textbf{0.9}                                      & 1.33                                              & 0.86                                               & 4                                               & 0.3                                                \\
                                 & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.94} & {\cellcolor[rgb]{0.937,0.937,0.937}}1.18          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.93           & {\cellcolor[rgb]{0.937,0.937,0.937}}2           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.83           \\
                                 & Test Suite 3                                     & 7                                               & 0.07                                              & \textbf{2.4}                                      & \textbf{0.73}                                      & 7                                               & 0.07                                               \\
                                 & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.94} & {\cellcolor[rgb]{0.937,0.937,0.937}}1.88          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.85           & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.94}  \\
                                 & Test Suite 5                                     & 5                                               & 0.1                                               & \textbf{2.35}                                     & \textbf{0.63}                                      & 5                                               & 0.1                                                \\
\hline
\end{tabular}
\end{table*}

\begin{table*}
\centering
\caption{Test prioritization on Planning module}
\begin{tabular}{l|lll} 
\hline
            & Baseline\_order & Baseline\_random & Proposed method  \\ 
\hline
Test suit 1 & 0.85            & 0.94             & \textbf{0.94}    \\ 
\hline
Test suit 2 & \textbf{0.97}   & 0.96             & \textbf{0.97}    \\ 
\hline
Test suit 3 & 0.69            & 0.78             & \textbf{0.81}    \\ 
\hline
Test suit 4 & 0.78            & \textbf{0.85}    & 0.78             \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\caption{Test prioritization on Signal detection}
\begin{tabular}{l|lll} 
\hline
            & Baseline\_order & Baseline\_random & Proposed method  \\ 
\hline
Test suit 1 & 0.87            & 0.88             & \textbf{0.91}    \\ 
\hline
Test suit 2 & \textbf{0.96}   & \textbf{0.96}    & \textbf{0.96}    \\ 
\hline
Test suit 3 & 0.74            & 0.83             & \textbf{0.88}    \\ 
\hline
Test suit 4 & 0.31            & \textbf{0.62}    & 0.17             \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\caption{Test prioritization on signal detection}
\begin{tabular}{c|l|llllll} 
\hline
\multirow{6}{*}{\textbf{Bug 1}} & \multirow{2}{*}{}                                & \multicolumn{2}{l|}{Baseline\_order}                                                                & \multicolumn{2}{l|}{Baseline\_random}                                                                & \multicolumn{2}{l}{Proposed method}                                                                  \\ 
\cline{3-8}
                                &                                                  & Top K                                           & AFPD                                              & Top K                                            & AFPD                                              & Top K                                           & AFPD                                               \\ 
\cline{2-8}
                                & Test Suite 1\textbf{ }                           & \textbf{1 }                                     & \textbf{0.94}                                     & 1.2                                              & 0.91                                              & \textbf{1 }                                     & \textbf{0.94}                                      \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1 } & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.88} & {\cellcolor[rgb]{0.937,0.937,0.937}}2.2          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.58          & {\cellcolor[rgb]{0.937,0.937,0.937}}2           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.63           \\
                                & Test Suite 3\textbf{ }                           & 2                                               & 0.75                                              & \textbf{1.7}                                     & \textbf{0.80}                                     & 2                                               & \textbf{0.75}                                      \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1 } & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.83} & {\cellcolor[rgb]{0.937,0.937,0.937}}2.9          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.60          & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1 } & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.83}  \\ 
\hline
\multirow{4}{*}{\textbf{Bug 2}} & Test Suite 1                                     & \textbf{1 }                                     & \textbf{0.98}                                     & 1.9                                              & 0.83                                              & \textbf{1 }                                     & \textbf{0.98}                                      \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}1           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.94          & {\cellcolor[rgb]{0.937,0.937,0.937}}1.2          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.82          & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.94}  \\
                                & Test Suite 3                                     & 2                                               & 0.79                                              & 1.1                                              & 0.90                                              & \textbf{1}                                      & \textbf{0.93}                                      \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}5           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.36          & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{2.1} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.74} & {\cellcolor[rgb]{0.937,0.937,0.937}}6           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.21           \\ 
\hline
\multirow{4}{*}{\textbf{Bug 3}} & Test Suite 1                                     & \textbf{1 }                                     & \textbf{0.94}                                     & 1.9                                              & 0.83                                              & \textbf{1 }                                     & \textbf{0.94}                                      \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 2 & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1 } & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.88} & {\cellcolor[rgb]{0.937,0.937,0.937}}2.0          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.63          & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.88}  \\
                                & Test Suite 3\textbf{ }                           & 3                                               & 0.58                                              & 1.2                                              & 0.89                                              & \textbf{1}                                      & \textbf{0.92}                                      \\
                                & {\cellcolor[rgb]{0.937,0.937,0.937}}Test Suite 4 & {\cellcolor[rgb]{0.937,0.937,0.937}}4           & {\cellcolor[rgb]{0.937,0.937,0.937}}0.41          & {\cellcolor[rgb]{0.937,0.937,0.937}}2.1          & {\cellcolor[rgb]{0.937,0.937,0.937}}0.73          & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{1}  & {\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{0.92}  \\
\hline
\end{tabular}
\end{table*}

\begin{table*}
\centering
\caption{Test length reduction strategy 1}
\begin{tabular}{lllll} 
\hline
\textbf{SUT}                                                                                                        & \textbf{Test suite} & \textbf{Total length} & \textbf{Reduced length} & \textbf{Reduction rate}  \\ 
\hline
\multirow{5}{*}{\textbf{Signal detection}}                                                                          & shalun              & 66.19                 & 25.5                    & 0.61                     \\
                                                                                                                    & san                 & 72.34                 & 42.66                   & 0.41                     \\
                                                                                                                    & gomentum            & 80.12                 & 20.41                   & 0.75                     \\
                                                                                                                    & cubetown            & 79.26                 & 20.54                   & 0.74                     \\
                                                                                                                    & total               & 297.91                & 109.1                   & 0.63                     \\ 
\hline
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & shalun              & 75.72                 & 17.64                   & 0.77                     \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & san                 & 110.71                & 60.75                   & 0.45                     \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & gomentum            & 93.06                 & 40.58                   & 0.56                     \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & cubetown            & 104.48                & 42.8                    & 0.59                     \\
\rowcolor[rgb]{0.937,0.937,0.937} \multirow{-5}{*}{{\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{Obstacle detection}} & total               & 383.96                & 161.77                  & 0.58                     \\ 
\hline
\multirow{5}{*}{\textbf{Planning }}                                                                                 & shalun              & 84.87                 & 38.71                   & 0.54                     \\
                                                                                                                    & san                 & 77.32                 & 42.32                   & 0.45                     \\
                                                                                                                    & gomentum            & 101.04                & 23.88                   & 0.76                     \\
                                                                                                                    & cubetown            & 94.1                  & 27.0                    & 0.71                     \\
                                                                                                                    & total               & 357.32                & 131.91                  & 0.63                     \\ 
\hline
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & shalun              & 46.03                 & 36.8                    & 0.2                      \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & san                 & 45.79                 & 30.98                   & 0.32                     \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & gomentum            & 83.5                  & 37.1                    & 0.56                     \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & cubetown            & 73.37                 & 47.33                   & 0.35                     \\
\rowcolor[rgb]{0.937,0.937,0.937} \multirow{-5}{*}{{\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{Prediction }}        & total               & 248.69                & 152.21                  & 0.39                     \\ 
\hline
\textbf{Total}                                                                                                      & total               & 1287.89               & 554.99                  & 0.57                     \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\caption{Test length reduction strategy 1 + strategy 2}
\begin{tabular}{l|llll} 
\hline
\textbf{SUT}                                                                                                        & \textbf{Test suite} & \textbf{Total length} & \textbf{Reduced length} & \textbf{Reduction rate}  \\ 
\hline
\multirow{5}{*}{\textbf{signal detection}}                                                                          & shalun              & 66.19                 & 10.5                    & 0.84                     \\
                                                                                                                    & san                 & 72.34                 & 13.83                   & 0.81                     \\
                                                                                                                    & gomentum            & 80.12                 & 11.41                   & 0.86                     \\
                                                                                                                    & cubetown            & 79.26                 & 15.0                    & 0.81                     \\
                                                                                                                    & total               & 297.91                & 50.74                   & 0.83                     \\ 
\hline
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & shalun              & 75.72                 & 5.64                    & 0.93                     \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & san                 & 110.71                & 43.47                   & 0.61                     \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & gomentum            & 93.06                 & 17.88                   & 0.81                     \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & cubetown            & 104.48                & 28.14                   & 0.73                     \\
\rowcolor[rgb]{0.937,0.937,0.937} \multirow{-5}{*}{{\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{obstacle detection}} & total               & 383.96                & 95.13                   & 0.75                     \\ 
\hline
\multirow{5}{*}{\textbf{planning }}                                                                                 & shalun              & 84.87                 & 18.0                    & 0.79                     \\
                                                                                                                    & san                 & 77.32                 & 10.61                   & 0.86                     \\
                                                                                                                    & gomentum            & 101.04                & 15.0                    & 0.85                     \\
                                                                                                                    & cubetown            & 94.1                  & 12.0                    & 0.87                     \\
                                                                                                                    & total               & 357.32                & 55.61                   & 0.84                     \\ 
\hline
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & shalun              & 46.03                 & 28.23                   & 0.39                     \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & san                 & 45.79                 & 30.98                   & 0.32                     \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & gomentum            & 83.5                  & 20.31                   & 0.76                     \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                              & cubetown            & 73.37                 & 41.94                   & 0.43                     \\
\rowcolor[rgb]{0.937,0.937,0.937} \multirow{-5}{*}{{\cellcolor[rgb]{0.937,0.937,0.937}}\textbf{prediction}}         & total               & 248.69                & 121.46                  & 0.51                     \\ 
\hline
\textbf{total}                                                                                                      & total               & 1287.89               & 322.93                  & 0.75                     \\
\hline
\end{tabular}
\end{table*}

\begin{table*}
\centering
\caption{Test effectiveness of reduced test set on signal detection system}
\begin{tabular}{ccccccc} 
\hline
Benchmarks (bugs)      & Test suite & TP & TN & FP & FN & F1 score  \\ 
\hline
\multirow{5}{*}{Bug 1} & shalun     & 4  & 5  & 0  & 1  & 0.89      \\
                       & san        & 6  & 9  & 1  & 0  & 0.92      \\
                       & gomentum   & 3  & 4  & 1  & 0  & 0.86      \\
                       & cubetown   & 1  & 6  & 0  & 1  & 0.67      \\
                       & total      & 14 & 24 & 2  & 2  & 0.88      \\ 
\hline
\multirow{5}{*}{Bug 2} & shalun     & 7  & 2  & 0  & 1  & 0.93      \\
                       & san        & 10 & 5  & 1  & 0  & 0.95      \\
                       & gomentum   & 5  & 2  & 0  & 1  & 0.91      \\
                       & cubetown   & 2  & 5  & 0  & 1  & 0.8       \\
                       & total      & 24 & 14 & 1  & 3  & 0.92      \\ 
\hline
\multirow{5}{*}{Bug 3} & shalun     & 7  & 2  & 0  & 1  & 0.93      \\
                       & san        & 11 & 4  & 1  & 0  & 0.96      \\
                       & gomentum   & 4  & 3  & 0  & 1  & 0.89      \\
                       & cubetown   & 2  & 5  & 0  & 1  & 0.8       \\
                       & total      & 24 & 14 & 1  & 3  & 0.92      \\ 
\hline
total                 & total      & 62 & 52 & 4  & 8  & 0.91      \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\caption{Test effectiveness of reduced test set on obstacle detection system}
\begin{tabular}{ccccccc} 
\hline
\textbf{Benchmarks (bugs)} & \textbf{Test suite} & \textbf{TP} & \textbf{TN} & \textbf{FP} & \textbf{FN} & \textbf{F1 score}  \\
\multirow{5}{*}{Bug 4}     & shalun              & 1           & 4           & 1           & 0           & 0.67               \\
                           & san                 & 2           & 18          & 1           & 0           & 0.8                \\
                           & gomentum            & 1           & 13          & 1           & 0           & 0.67               \\
                           & cubetown            & 3           & 12          & 1           & 0           & 0.86               \\
                           & total               & 7           & 47          & 4           & 0           & 0.78               \\ 
\hline
\multirow{5}{*}{Bug 5}     & shalun              & 0           & 6           & 1           & 0           & 0.0                \\
                           & san                 & 2           & 18          & 1           & 0           & 0.8                \\
                           & gomentum            & 1           & 14          & 1           & 0           & 0.67               \\
                           & cubetown            & 4           & 11          & 1           & 0           & 0.89               \\
                           & total               & 7           & 49          & 4           & 0           & 0.78               \\ 
\hline
\multirow{5}{*}{Bug 6}     & shalun              & 0           & 5           & 1           & 0           & 0.0                \\
                           & san                 & 2           & 18          & 1           & 0           & 0.8                \\
                           & gomentum            & 1           & 14          & 1           & 0           & 0.67               \\
                           & cubetown            & 3           & 12          & 1           & 0           & 0.86               \\
                           & total               & 6           & 49          & 4           & 0           & 0.75               \\ 
\hline
\multirow{5}{*}{Bug 7}     & shalun              & 0           & 6           & 1           & 0           & 0.0                \\
                           & san                 & 2           & 18          & 1           & 0           & 0.8                \\
                           & gomentum            & 1           & 14          & 1           & 0           & 0.67               \\
                           & cubetown            & 4           & 11          & 1           & 0           & 0.89               \\
                           & total               & 7           & 49          & 4           & 0           & 0.78               \\ 
\hline
\multirow{5}{*}{Bug 8}     & shalun              & 0           & 6           & 1           & 0           & 0.0                \\
                           & san                 & 2           & 18          & 1           & 0           & 0.8                \\
                           & gomentum            & 1           & 14          & 1           & 0           & 0.67               \\
                           & cubetown            & 3           & 12          & 1           & 0           & 0.86               \\
                           & total               & 6           & 50          & 4           & 0           & 0.75               \\ 
\hline
\multirow{5}{*}{Bug 9}     & shalun              & 0           & 6           & 1           & 0           & 0.0                \\
                           & san                 & 3           & 18          & 1           & 0           & 0.86               \\
                           & gomentum            & 2           & 13          & 1           & 0           & 0.8                \\
                           & cubetown            & 4           & 11          & 1           & 0           & 0.89               \\
                           & total               & 9           & 48          & 4           & 0           & 0.82               \\ 
\hline
total                      & total               & 42          & 292         & 24          & 0           & 0.78               \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\caption{Test effectiveness of reduced test set on planning system}
\begin{tabular}{ccccccc} 
\hline
\textbf{Benchmarks (bugs)} & \textbf{Test suite} & \textbf{TP} & \textbf{TN} & \textbf{FP} & \textbf{FN} & \textbf{F1 score}  \\ 
\hline
\multirow{5}{*}{Bug 10}    & shalun              & 7           & 5           & 0           & 1           & 0.93               \\
                           & san                 & 2           & 11          & 1           & 0           & 0.8                \\
                           & gomentum            & 0           & 8           & 1           & 0           & 0.0                \\
                           & cubetown            & 0           & 8           & 1           & 0           & 0.0                \\
                           & total               & 9           & 32          & 3           & 1           & 0.82               \\ 
\hline
\multirow{5}{*}{Bug 11}    & shalun              & 2           & 10          & 1           & 0           & 0.8                \\
                           & san                 & 4           & 10          & 0           & 1           & 0.89               \\
                           & gomentum            & 0           & 8           & 1           & 0           & 0.0                \\
                           & cubetown            & 3           & 6           & 1           & 0           & 0.86               \\
                           & total               & 9           & 34          & 3           & 1           & 0.82               \\ 
\hline
\multirow{5}{*}{Bug 12}    & shalun              & 3           & 10          & 1           & 0           & 0.86               \\
                           & san                 & 7           & 7           & 0           & 1           & 0.93               \\
                           & gomentum            & 1           & 7           & 1           & 0           & 0.67               \\
                           & cubetown            & 5           & 4           & 1           & 0           & 0.91               \\
                           & total               & 16          & 28          & 3           & 1           & 0.89               \\ 
\hline
\multirow{5}{*}{Bug 13}    & shalun              & 9           & 2           & 1           & 0           & 0.95               \\
                           & san                 & 4           & 11          & 1           & 0           & 0.89               \\
                           & gomentum            & 2           & 6           & 1           & 0           & 0.8                \\
                           & cubetown            & 3           & 6           & 1           & 0           & 0.86               \\
                           & total               & 18          & 25          & 4           & 0           & 0.9                \\ 
\hline
total                      & total               & 52          & 119         & 13          & 3           & 0.87               \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\caption{Test effectiveness of reduced test set on prediction system}
\begin{tabular}{ccccccc} 
\hline
\textbf{Benchmarks (bugs)} & \textbf{Test suite} & \textbf{TP} & \textbf{TN} & \textbf{FP} & \textbf{FN} & \textbf{F1 score}  \\
\multirow{5}{*}{Bug 14}    & shalun              & 0           & 13          & 1           & 0           & 0.0                \\
                           & san                 & 0           & 11          & 1           & 0           & 0.0                \\
                           & gomentum            & 0           & 13          & 1           & 0           & 0.0                \\
                           & cubetown            & 2           & 16          & 1           & 0           & 0.8                \\
                           & total               & 2           & 53          & 4           & 0           & 0.5                \\ 
\hline
\multirow{5}{*}{Bug 15}    & shalun              & 0           & 13          & 1           & 0           & 0.0                \\
                           & san                 & 1           & 9           & 1           & 0           & 0.67               \\
                           & gomentum            & 1           & 12          & 1           & 0           & 0.67               \\
                           & cubetown            & 3           & 15          & 1           & 0           & 0.86               \\
                           & total               & 5           & 49          & 4           & 0           & 0.71               \\ 
\hline
\multirow{5}{*}{Bug 16}    & shalun              & 0           & 13          & 1           & 0           & 0.0                \\
                           & san                 & 1           & 10          & 1           & 0           & 0.67               \\
                           & gomentum            & 0           & 13          & 1           & 0           & 0.0                \\
                           & cubetown            & 1           & 17          & 1           & 0           & 0.67               \\
                           & total               & 2           & 53          & 4           & 0           & 0.5                \\ 
\hline
total                      & total               & 9           & 155         & 12          & 0           & 0.6                \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\caption{Test effectiveness of reduced test set on signal detection system, setting 2}
\begin{tabular}{ccccccccc} 
\hline
\textbf{Benchmarks (bugs)} & \textbf{Test suite} & \textbf{Total bugs} & \textbf{Covered bugs} & \textbf{TP} & \textbf{TN} & \textbf{FP} & \textbf{FN} & \textbf{F1 score}  \\ 
\hline
\multirow{5}{*}{Bug 1}     & shalun              & 2                   & 1                     & 1           & 3           & 1           & 0           & 0.67               \\
                           & san                 & 3                   & 2                     & 2           & 3           & 1           & 0           & 0.8                \\
                           & gomentum            & 3                   & 3                     & 3           & 1           & 1           & 0           & 0.86               \\
                           & cubetown            & 1                   & 0                     & 0           & 5           & 1           & 0           & 0.0                \\
                           & total               & 9                   & 6                     & 6           & 12          & 4           & 0           & 0.75               \\ 
\hline
\multirow{5}{*}{Bug 2}     & shalun              & 3                   & 3                     & 3           & 1           & 0           & 1           & 0.86               \\
                           & san                 & 5                   & 4                     & 4           & 3           & 1           & 0           & 0.89               \\
                           & gomentum            & 5                   & 5                     & 5           & 1           & 0           & 1           & 0.91               \\
                           & cubetown            & 2                   & 2                     & 2           & 3           & 0           & 1           & 0.8                \\
                           & total               & 15                  & 14                    & 14          & 8           & 1           & 3           & 0.88               \\ 
\hline
\multirow{5}{*}{Bug 3}     & shalun              & 4                   & 4                     & 4           & 1           & 0           & 1           & 0.89               \\
                           & san                 & 5                   & 4                     & 4           & 3           & 1           & 0           & 0.89               \\
                           & gomentum            & 4                   & 4                     & 4           & 2           & 0           & 1           & 0.89               \\
                           & cubetown            & 2                   & 2                     & 2           & 4           & 0           & 1           & 0.8                \\
                           & total               & 15                  & 14                    & 14          & 10          & 1           & 3           & 0.88               \\ 
\hline
signal                     & total               & 39                  & 34                    & 34          & 30          & 6           & 6           & 0.85               \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\caption{Test effectiveness of reduced test set on obstacle detection system, setting 2}
\begin{tabular}{ccccccccc} 
\hline
\textbf{Benchmarks (bugs)} & \textbf{Test suite} & \textbf{Total bugs} & \textbf{Covered bugs} & \textbf{TP} & \textbf{TN} & \textbf{FP} & \textbf{FN} & \textbf{F1 score}  \\ 
\hline
\multirow{5}{*}{Bug 4}     & shalun              & 2                   & 1                     & 1           & 0           & 0           & 1           & 0.67               \\
                           & san                 & 4                   & 1                     & 1           & 12          & 1           & 0           & 0.67               \\
                           & gomentum            & 1                   & 0                     & 0           & 5           & 1           & 0           & 0.0                \\
                           & cubetown            & 3                   & 2                     & 2           & 8           & 1           & 0           & 0.8                \\
                           & total               & 10                  & 4                     & 4           & 25          & 3           & 1           & 0.67               \\ 
\hline
\multirow{5}{*}{Bug 5}     & shalun              & 0                   & 0                     & 0           & 2           & 1           & 0           & 0.0                \\
                           & san                 & 4                   & 1                     & 1           & 12          & 1           & 0           & 0.67               \\
                           & gomentum            & 2                   & 1                     & 1           & 6           & 1           & 0           & 0.67               \\
                           & cubetown            & 4                   & 3                     & 3           & 8           & 1           & 0           & 0.86               \\
                           & total               & 10                  & 5                     & 5           & 28          & 4           & 0           & 0.71               \\ 
\hline
\multirow{5}{*}{Bug 6}     & shalun              & 1                   & 0                     & 0           & 1           & 1           & 0           & 0.0                \\
                           & san                 & 4                   & 1                     & 1           & 12          & 1           & 0           & 0.67               \\
                           & gomentum            & 2                   & 1                     & 1           & 6           & 1           & 0           & 0.67               \\
                           & cubetown            & 3                   & 2                     & 2           & 8           & 1           & 0           & 0.8                \\
                           & total               & 10                  & 4                     & 4           & 27          & 4           & 0           & 0.67               \\ 
\hline
\multirow{5}{*}{Bug 7}     & shalun              & 0                   & 0                     & 0           & 2           & 1           & 0           & 0.0                \\
                           & san                 & 4                   & 1                     & 1           & 12          & 1           & 0           & 0.67               \\
                           & gomentum            & 2                   & 1                     & 1           & 6           & 1           & 0           & 0.67               \\
                           & cubetown            & 4                   & 3                     & 3           & 8           & 1           & 0           & 0.86               \\
                           & total               & 10                  & 5                     & 5           & 28          & 4           & 0           & 0.71               \\ 
\hline
\multirow{5}{*}{Bug 8}     & shalun              & 0                   & 0                     & 0           & 2           & 1           & 0           & 0.0                \\
                           & san                 & 4                   & 1                     & 1           & 12          & 1           & 0           & 0.67               \\
                           & gomentum            & 2                   & 1                     & 1           & 6           & 1           & 0           & 0.67               \\
                           & cubetown            & 3                   & 2                     & 2           & 8           & 1           & 0           & 0.8                \\
                           & total               & 9                   & 4                     & 4           & 28          & 4           & 0           & 0.67               \\ 
\hline
\multirow{5}{*}{Bug 9}     & shalun              & 0                   & 0                     & 0           & 2           & 1           & 0           & 0.0                \\
                           & san                 & 4                   & 2                     & 2           & 11          & 1           & 0           & 0.8                \\
                           & gomentum            & 3                   & 2                     & 2           & 5           & 1           & 0           & 0.8                \\
                           & cubetown            & 4                   & 3                     & 3           & 8           & 1           & 0           & 0.86               \\
                           & total               & 11                  & 7                     & 7           & 26          & 4           & 0           & 0.78               \\ 
\hline
total                      & total               & 60                  & 29                    & 29          & 162         & 23          & 1           & 0.71               \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\caption{Test effectiveness of reduced test set on planning system, setting 2}
\begin{tabular}{ccccccccc} 
\hline
\textbf{Benchmarks (bugs)} & \textbf{Test suite} & \textbf{Total bugs} & \textbf{Covered bugs} & \textbf{TP} & \textbf{TN} & \textbf{FP} & \textbf{FN} & \textbf{F1 score}  \\ 
\hline
\multirow{5}{*}{Bug 10}    & shalun              & 4                   & 4                     & 4           & 2           & 0           & 1           & 0.89               \\
                           & san                 & 1                   & 0                     & 0           & 4           & 1           & 0           & 0.0                \\
                           & gomentum            & 0                   & 0                     & 0           & 5           & 1           & 0           & 0.0                \\
                           & cubetown            & 1                   & 0                     & 0           & 3           & 1           & 0           & 0.0                \\
                           & total               & 6                   & 4                     & 4           & 14          & 3           & 1           & 0.67               \\ 
\hline
\multirow{5}{*}{Bug 11}    & shalun              & 1                   & 0                     & 0           & 5           & 1           & 0           & 0.0                \\
                           & san                 & 2                   & 0                     & 0           & 4           & 1           & 0           & 0.0                \\
                           & gomentum            & 0                   & 0                     & 0           & 5           & 1           & 0           & 0.0                \\
                           & cubetown            & 3                   & 2                     & 2           & 4           & 1           & 0           & 0.8                \\
                           & total               & 6                   & 2                     & 2           & 18          & 4           & 0           & 0.5                \\ 
\hline
\multirow{5}{*}{Bug 12}    & shalun              & 2                   & 0                     & 0           & 5           & 1           & 0           & 0.0                \\
                           & san                 & 1                   & 1                     & 1           & 2           & 1           & 0           & 0.67               \\
                           & gomentum            & 1                   & 0                     & 0           & 4           & 1           & 0           & 0.0                \\
                           & cubetown            & 4                   & 3                     & 3           & 3           & 1           & 0           & 0.86               \\
                           & total               & 8                   & 4                     & 4           & 14          & 4           & 0           & 0.67               \\ 
\hline
\multirow{5}{*}{Bug 13~}   & shalun              & 5                   & 5                     & 5           & 1           & 1           & 0           & 0.91               \\
                           & san                 & 2                   & 1                     & 1           & 2           & 1           & 0           & 0.67               \\
                           & gomentum            & 2                   & 2                     & 2           & 5           & 1           & 0           & 0.8                \\
                           & cubetown            & 3                   & 1                     & 1           & 4           & 1           & 0           & 0.67               \\
                           & total               & 12                  & 9                     & 9           & 12          & 4           & 0           & 0.82               \\ 
\hline
total                      & total               & 32                  & 19                    & 19          & 58          & 15          & 1           & 0.7                \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\caption{Test effectiveness of reduced test set on prediction system, setting 2}
\begin{tabular}{ccccccccc} 
\hline
\textbf{Benchmarks (bugs)} & \textbf{Test suite} & \textbf{Total bugs} & \textbf{Covered bugs} & \textbf{TP} & \textbf{TN} & \textbf{FP} & \textbf{FN} & \textbf{F1 score}  \\ 
\hline
\multirow{5}{*}{Bug 14}    & shalun              & 0                   & 0                     & 0           & 10          & 1           & 0           & 0.0                \\
                           & san                 & 0                   & 0                     & 0           & 11          & 1           & 0           & 0.0                \\
                           & gomentum            & 0                   & 0                     & 0           & 7           & 1           & 0           & 0.0                \\
                           & cubetown            & 2                   & 1                     & 1           & 15          & 1           & 0           & 0.67               \\
                           & total               & 2                   & 1                     & 1           & 43          & 4           & 0           & 0.33               \\ 
\hline
\multirow{5}{*}{Bug 15}    & shalun              & 0                   & 0                     & 0           & 10          & 1           & 0           & 0.0                \\
                           & san                 & 2                   & 1                     & 1           & 9           & 1           & 0           & 0.67               \\
                           & gomentum            & 1                   & 1                     & 1           & 6           & 1           & 0           & 0.67               \\
                           & cubetown            & 3                   & 2                     & 2           & 14          & 1           & 0           & 0.8                \\
                           & total               & 6                   & 4                     & 4           & 39          & 4           & 0           & 0.67               \\ 
\hline
\multirow{5}{*}{Bug 16}    & shalun              & 0                   & 0                     & 0           & 10          & 1           & 0           & 0.0                \\
                           & san                 & 1                   & 1                     & 1           & 10          & 1           & 0           & 0.67               \\
                           & gomentum            & 0                   & 0                     & 0           & 7           & 1           & 0           & 0.0                \\
                           & cubetown            & 1                   & 1                     & 1           & 15          & 1           & 0           & 0.67               \\
                           & total               & 2                   & 2                     & 2           & 42          & 4           & 0           & 0.5                \\ 
\hline
total                      & total               & 10                  & 7                     & 7           & 124         & 12          & 0           & 0.54               \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\begin{tabular}{llllllll} 
\hline
Benchmarks (bugs) & Test suite & Baseline 1 Top K & Baseline 1 APFD & Baseline 2 Top K & Baseline 2 APFD & Proposed method Top K & Proposed method APFD  \\
Bug 1             & shalun     & 3                & 0.72            & 3.0              & 0.72            & 5                     & 0.5                   \\
Bug 1             & san        & 2                & 0.9             & 2.0              & 0.9             & 1                     & 0.97                  \\
Bug 1             & gomentum   & 2                & 0.79            & 2.0              & 0.79            & 1                     & 0.93                  \\
Bug 1             & cubetown   & 2                & 0.79            & 2.0              & 0.79            & 4                     & 0.5                   \\
Bug 1             & total      & 2.25             & 0.8             & 2.25             & 0.8             & 2.75                  & 0.72                  \\ 
\hline
Bug 2             & shalun     & 1                & 0.94            & 1.0              & 0.94            & 1                     & 0.94                  \\
Bug 2             & san        & 1                & 0.97            & 1.0              & 0.97            & 1                     & 0.97                  \\
Bug 2             & gomentum   & 2                & 0.79            & 1.0              & 0.93            & 1                     & 0.93                  \\
Bug 2             & cubetown   & 2                & 0.79            & 1.0              & 0.93            & 3                     & 0.64                  \\
Bug 2             & total      & 1.5              & 0.87            & 1.0              & 0.94            & 1.5                   & 0.87                  \\ 
\hline
Bug 3             & shalun     & 1                & 0.94            & 2.0              & 0.83            & 1                     & 0.94                  \\
Bug 3             & san        & 1                & 0.97            & 1.0              & 0.97            & 1                     & 0.97                  \\
Bug 3             & gomentum   & 3                & 0.64            & 1.0              & 0.93            & 1                     & 0.93                  \\
Bug 3             & cubetown   & 2                & 0.79            & 6.0              & 0.21            & 1                     & 0.93                  \\
Bug 3             & total      & 1.75             & 0.83            & 2.5              & 0.73            & 1.0                   & 0.94                  \\
total             & total      & 1.83             & 0.84            & 1.92             & 0.83            & 1.75                  & 0.85                  \\ 
\hline
Bug 4             & shalun     & 2                & 0.75            & 6.0              & 0.08            & 4                     & 0.42                  \\
Bug 4             & san        & 8                & 0.66            & 1.0              & 0.98            & 6                     & 0.75                  \\
Bug 4             & gomentum   & 7                & 0.57            & 9.0              & 0.43            & 7                     & 0.57                  \\
Bug 4             & cubetown   & 1                & 0.97            & 3.0              & 0.83            & 2                     & 0.9                   \\
Bug 4             & total      & 4.5              & 0.74            & 4.75             & 0.58            & 4.75                  & 0.66                  \\ 
\hline
Bug 5             & shalun     & -1               & -1.0            & -1.0             & -1.0            & -1                    & -1.0                  \\
Bug 5             & san        & 8                & 0.66            & 1.0              & 0.98            & 6                     & 0.75                  \\
Bug 5             & gomentum   & 7                & 0.59            & 8.0              & 0.53            & 5                     & 0.72                  \\
Bug 5             & cubetown   & 1                & 0.97            & 1.0              & 0.97            & 2                     & 0.9                   \\
Bug 5             & total      & 5.33             & 0.74            & 3.33             & 0.83            & 4.33                  & 0.79                  \\ 
\hline
Bug 6             & shalun     & -1               & -1.0            & -1.0             & -1.0            & -1                    & -1.0                  \\
Bug 6             & san        & 8                & 0.66            & 13.0             & 0.43            & 6                     & 0.75                  \\
Bug 6             & gomentum   & 7                & 0.59            & 15.0             & 0.09            & 5                     & 0.72                  \\
Bug 6             & cubetown   & 1                & 0.97            & 7.0              & 0.57            & 2                     & 0.9                   \\
Bug 6             & total      & 5.33             & 0.74            & 11.67            & 0.36            & 4.33                  & 0.79                  \\ 
\hline
Bug 7             & shalun     & -1               & -1.0            & -1.0             & -1.0            & -1                    & -1.0                  \\
Bug 7             & san        & 8                & 0.66            & 7.0              & 0.7             & 6                     & 0.75                  \\
Bug 7             & gomentum   & 7                & 0.59            & 9.0              & 0.47            & 5                     & 0.72                  \\
Bug 7             & cubetown   & 1                & 0.97            & 3.0              & 0.83            & 2                     & 0.9                   \\
Bug 7             & total      & 5.33             & 0.74            & 6.33             & 0.67            & 4.33                  & 0.79                  \\ 
\hline
Bug 8             & shalun     & -1               & -1.0            & -1.0             & -1.0            & -1                    & -1.0                  \\
Bug 8             & san        & 8                & 0.66            & 3.0              & 0.89            & 6                     & 0.75                  \\
Bug 8             & gomentum   & 7                & 0.59            & 13.0             & 0.22            & 5                     & 0.72                  \\
Bug 8             & cubetown   & 1                & 0.97            & 6.0              & 0.63            & 2                     & 0.9                   \\
Bug 8             & total      & 5.33             & 0.74            & 7.33             & 0.58            & 4.33                  & 0.79                  \\ 
\hline
Bug 9             & shalun     & -1               & -1.0            & -1.0             & -1.0            & -1                    & -1.0                  \\
Bug 9             & san        & 8                & 0.66            & 2.0              & 0.93            & 6                     & 0.75                  \\
Bug 9             & gomentum   & 7                & 0.59            & 4.0              & 0.78            & 3                     & 0.84                  \\
Bug 9             & cubetown   & 1                & 0.97            & 4.0              & 0.77            & 2                     & 0.9                   \\
Bug 9             & total      & 5.33             & 0.74            & 3.33             & 0.83            & 3.67                  & 0.83                  \\
total             & total      & 5.16             & 0.74            & 6.05             & 0.64            & 4.32                  & 0.77                  \\ 
\hline
Bug 10            & shalun     & 3                & 0.81            & 2.0              & 0.88            & 1                     & 0.96                  \\
Bug 10            & san        & 7                & 0.57            & 6.0              & 0.63            & 8                     & 0.5                   \\
Bug 10            & gomentum   & -1               & -1.0            & -1.0             & -1.0            & -1                    & -1.0                  \\
Bug 10            & cubetown   & -1               & -1.0            & -1.0             & -1.0            & -1                    & -1.0                  \\
Bug 10            & total      & 5.0              & 0.69            & 4.0              & 0.76            & 4.5                   & 0.73                  \\ 
\hline
Bug 11            & shalun     & 3                & 0.81            & 1.0              & 0.96            & 3                     & 0.81                  \\
Bug 11            & san        & 3                & 0.83            & 2.0              & 0.9             & 5                     & 0.7                   \\
Bug 11            & gomentum   & -1               & -1.0            & -1.0             & -1.0            & -1                    & -1.0                  \\
Bug 11            & cubetown   & 1                & 0.94            & 1.0              & 0.94            & 1                     & 0.94                  \\
Bug 11            & total      & 2.33             & 0.86            & 1.33             & 0.93            & 3.0                   & 0.82                  \\ 
\hline
Bug 12            & shalun     & 3                & 0.81            & 1.0              & 0.96            & 3                     & 0.81                  \\
Bug 12            & san        & 1                & 0.96            & 3.0              & 0.82            & 3                     & 0.82                  \\
Bug 12            & gomentum   & 4                & 0.56            & 5.0              & 0.44            & 5                     & 0.44                  \\
Bug 12            & cubetown   & 1                & 0.94            & 3.0              & 0.72            & 1                     & 0.94                  \\
Bug 12            & total      & 2.25             & 0.82            & 3.0              & 0.73            & 3.0                   & 0.75                  \\ 
\hline
Bug 13            & shalun     & 1                & 0.96            & 4.0              & 0.73            & 3                     & 0.81                  \\
Bug 13            & san        & 5                & 0.7             & 1.0              & 0.97            & 8                     & 0.5                   \\
Bug 13            & gomentum   & 7                & 0.19            & 1.0              & 0.94            & 2                     & 0.81                  \\
Bug 13            & cubetown   & 1                & 0.94            & 5.0              & 0.5             & 1                     & 0.94                  \\
Bug 13            & total      & 3.5              & 0.7             & 2.75             & 0.78            & 3.5                   & 0.77                  \\ 
\hline
total             & total      & 3.08             & 0.77            & 2.69             & 0.8             & 3.38                  & 0.77                  \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\begin{tabular}{ccccc} 
\hline
\multicolumn{1}{l}{\textbf{Benchmarks (bugs)}} & \multicolumn{1}{l}{\textbf{Test suite}} & \multicolumn{1}{l}{\textbf{Baseline 1 test length}} & \multicolumn{1}{l}{\textbf{Baseline 2 test length}} & \multicolumn{1}{l}{\textbf{Proposed method test length}}  \\ 
\hline
\multirow{4}{*}{Bug 1}                         & shalun                                  & 25.6                                                & \textbf{10.3}                                       & 14.1                                                      \\
                                               & san                                     & 6.03                                                & 7.81                                                & \textbf{3.0}                                              \\
                                               & gomentum                                & 2.41                                                & 28.19                                               & \textbf{2.41}                                             \\
                                               & cubetown                                & 79.26                                               & 44.47                                               & \textbf{11.89}                                            \\ 
\hline
\multirow{4}{*}{Bug 2}                         & shalun                                  & 17.14                                               & 9.34                                                & \textbf{3.0}                                              \\
                                               & san                                     & 6.03                                                & 5.99                                                & \textbf{2.39}                                             \\
                                               & gomentum                                & \textbf{2.41}                                       & 13.7                                                & 3.0                                                       \\
                                               & cubetown                                & \textbf{8.25}                                       & 31.11                                               & 8.89                                                      \\ 
\hline
\multirow{4}{*}{Bug 3}                         & shalun                                  & 17.14                                               & 7.42                                                & \textbf{2.46}                                             \\
                                               & san                                     & 6.03                                                & 6.54                                                & \textbf{3.0}                                              \\
                                               & gomentum                                & \textbf{2.41}                                       & 17.06                                               & \textbf{2.41}                                             \\
                                               & cubetown                                & 8.25                                                & 26.73                                               & \textbf{2.89}                                             \\ 
\hline
\multirow{4}{*}{Bug 4}                         & shalun                                  & 57.64                                               & 34.25                                               & \textbf{11.64}                                            \\
                                               & san                                     & 77.79                                               & 45.54                                               & \textbf{17.36}                                            \\
                                               & gomentum                                & 67.86                                               & 48.74                                               & \textbf{19.71}                                            \\
                                               & cubetown                                & 6.98                                                & 37.89                                               & \textbf{6.0}                                              \\ 
\hline
\multirow{4}{*}{Bug 5}                         & shalun                                  & -1.0                                                & -1.0                                                & -1.0                                                      \\
                                               & san                                     & 77.79                                               & 20.39                                               & \textbf{17.36}                                            \\
                                               & gomentum                                & 71.47                                               & 47.14                                               & \textbf{13.71}                                            \\
                                               & cubetown                                & 6.98                                                & 12.29                                               & \textbf{6.0}                                              \\ 
\hline
\multirow{4}{*}{Bug 6}                         & shalun                                  & -1.0                                                & -1.0                                                & -1.0                                                      \\
                                               & san                                     & 77.79                                               & 45.64                                               & \textbf{17.36}                                            \\
                                               & gomentum                                & 71.47                                               & 61.95                                               & \textbf{13.71}                                            \\
                                               & cubetown                                & 6.98                                                & 25.34                                               & \textbf{6.0}                                              \\ 
\hline
\multirow{4}{*}{Bug 7}                         & shalun                                  & -1.0                                                & -1.0                                                & -1.0                                                      \\
                                               & san                                     & 77.79                                               & 31.79                                               & \textbf{17.36}                                            \\
                                               & gomentum                                & 71.47                                               & 50.66                                               & \textbf{13.71}                                            \\
                                               & cubetown                                & 6.98                                                & 29.66                                               & \textbf{6.0}                                              \\ 
\hline
\multirow{4}{*}{Bug 8}                         & shalun                                  & -1.0                                                & -1.0                                                & -1.0                                                      \\
                                               & san                                     & 77.79                                               & 38.38                                               & \textbf{17.36}                                            \\
                                               & gomentum                                & 71.47                                               & 53.98                                               & \textbf{13.71}                                            \\
                                               & cubetown                                & 6.98                                                & 28.11                                               & \textbf{6.0}                                              \\ 
\hline
\multirow{4}{*}{Bug 9}                         & shalun                                  & -1.0                                                & -1.0                                                & -1.0                                                      \\
                                               & san                                     & 18.61                                               & 25.63                                               & \textbf{17.36}                                            \\
                                               & gomentum                                & 35.37                                               & 35.37                                               & \textbf{8.27}                                             \\
                                               & cubetown                                & 6.98                                                & 39.6                                                & \textbf{6.0}                                              \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\begin{tabular}{ccccc} 
\hline
\multicolumn{1}{l}{\textbf{Benchmarks (bugs)}} & \multicolumn{1}{l}{\textbf{Test suite}} & \multicolumn{1}{l}{\textbf{Baseline 1 test length}} & \multicolumn{1}{l}{\textbf{Baseline 2 test length}} & \multicolumn{1}{l}{\textbf{Proposed method test length}}  \\ 
\hline
\multirow{4}{*}{Bug 10}                        & shalun                                  & 11.72                                               & 8.89                                                & \textbf{3.0}                                              \\
                                               & san                                     & 17.88                                               & \textbf{13.68}                                      & 23.16                                                     \\
                                               & gomentum                                & -1.0                                                & -1.0                                                & -1.0                                                      \\
                                               & cubetown                                & -1.0                                                & -1.0                                                & -1.0                                                      \\ 
\hline
\multirow{4}{*}{Bug 11}                        & shalun                                  & 43.82                                               & 34.21                                               & \textbf{9.0}                                              \\
                                               & san                                     & 17.88                                               & 20.12                                               & \textbf{14.16}                                            \\
                                               & gomentum                                & -1.0                                                & -1.0                                                & -1.0                                                      \\
                                               & cubetown                                & 4.1                                                 & 21.41                                               & \textbf{3.0}                                              \\ 
\hline
\multirow{4}{*}{Bug 12}                        & shalun                                  & 43.82                                               & 22.86                                               & \textbf{9.0}                                              \\
                                               & san                                     & \textbf{7.02}                                       & 10.48                                               & 9.0                                                       \\
                                               & gomentum                                & 72.08                                               & 64.13                                               & \textbf{15.0}                                             \\
                                               & cubetown                                & 4.1                                                 & 18.24                                               & \textbf{3.0}                                              \\ 
\hline
\multirow{4}{*}{Bug 13}                        & shalun                                  & \textbf{5.18}                                       & 6.28                                                & 9.0                                                       \\
                                               & san                                     & \textbf{17.88}                                      & 20.18                                               & 23.16                                                     \\
                                               & gomentum                                & 50.96                                               & 40.58                                               & \textbf{6.0}                                              \\
                                               & cubetown                                & 4.1                                                 & 18.98                                               & \textbf{3.0}                                              \\
\hline
\end{tabular}
\end{table*}

\begin{table*}
\centering
\begin{tabular}{llllllll} 
\hline
\multirow{2}{*}{\textbf{Benchmarks (bugs)}} & \multirow{2}{*}{\textbf{Test suite}} & \multicolumn{2}{l}{\textbf{Baseline 1}} & \multicolumn{2}{l}{\textbf{Baseline 2}} & \multicolumn{2}{l}{\textbf{Proposed method~}}  \\
                                            &                                      & Top K         & AFPD                    & Top K & AFPD                            & Top K         & AFPD                           \\ 
\hline
\multirow{5}{*}{Bug 1}                      & shalun                               & 3             & 0.72                    & 2.1   & 0.82                            & 5             & 0.5                            \\
                                            & san                                  & 2             & 0.9                     & 2.5   & 0.87                            & 1             & 0.97                           \\
                                            & gomentum                             & 2             & 0.79                    & 2.7   & 0.69                            & 1             & 0.93                           \\
                                            & cubetown                             & 2             & 0.79                    & 3.7   & 0.55                            & 4             & 0.5                            \\
                                            & total                                & \textbf{2.25} & \textbf{0.8}            & 2.75  & 0.73                            & 2.75          & 0.72                           \\ 
\hline
\multirow{5}{*}{Bug 2}                      & shalun                               & 1             & 0.94                    & 1.3   & 0.91                            & 1             & 0.94                           \\
                                            & san                                  & 1             & 0.97                    & 1.4   & 0.94                            & 1             & 0.97                           \\
                                            & gomentum                             & 2             & 0.79                    & 1.1   & 0.92                            & 1             & 0.93                           \\
                                            & cubetown                             & 2             & 0.79                    & 2.9   & 0.66                            & 3             & 0.64                           \\
                                            & total                                & 1.5           & 0.87                    & 1.68  & 0.86                            & \textbf{1.5}  & \textbf{0.87}                  \\ 
\hline
\multirow{5}{*}{Bug 3}                      & shalun                               & 1             & 0.94                    & 1.2   & 0.92                            & 1             & 0.94                           \\
                                            & san                                  & 1             & 0.97                    & 1.1   & 0.96                            & 1             & 0.97                           \\
                                            & gomentum                             & 3             & 0.64                    & 1.7   & 0.83                            & 1             & 0.93                           \\
                                            & cubetown                             & 2             & 0.79                    & 3.0   & 0.65                            & 1             & 0.93                           \\
                                            & total                                & 1.75          & 0.83                    & 1.75  & 0.84                            & \textbf{1.0}  & \textbf{0.94}                  \\ 
\hline
\textbf{Siginal total}                      & total                                & 1.83          & 0.84                    & 2.06  & 0.81                            & \textbf{1.75} & \textbf{0.85}                  \\ 
\hline
\multirow{5}{*}{Bug 4}                      & shalun                               & 2             & 0.75                    & 3.1   & 0.57                            & 4             & 0.42                           \\
                                            & san                                  & 8             & 0.66                    & 8.1   & 0.66                            & 6             & 0.75                           \\
                                            & gomentum                             & 7             & 0.57                    & 7.8   & 0.51                            & 7             & 0.57                           \\
                                            & cubetown                             & 1             & 0.97                    & 3.0   & 0.83                            & 2             & 0.9                            \\
                                            & total                                & \textbf{4.5}  & \textbf{0.74}           & 5.5   & 0.64                            & 4.75          & 0.66                           \\ 
\hline
\multirow{5}{*}{Bug 5}                      & shalun                               & -1            & -1.0                    & -1.0  & -1.0                            & -1            & -1.0                           \\
                                            & san                                  & 8             & 0.66                    & 11.3  & 0.51                            & 6             & 0.75                           \\
                                            & gomentum                             & 7             & 0.59                    & 7.4   & 0.57                            & 5             & 0.72                           \\
                                            & cubetown                             & 1             & 0.97                    & 2.9   & 0.84                            & 2             & 0.9                            \\
                                            & total                                & 5.33          & 0.74                    & 7.2   & 0.64                            & \textbf{4.33} & \textbf{0.79}                  \\ 
\hline
\multirow{5}{*}{Bug 6}                      & shalun                               & -1            & -1.0                    & -1.0  & -1.0                            & -1            & -1.0                           \\
                                            & san                                  & 8             & 0.66                    & 9.4   & 0.59                            & 6             & 0.75                           \\
                                            & gomentum                             & 7             & 0.59                    & 7.1   & 0.59                            & 5             & 0.72                           \\
                                            & cubetown                             & 1             & 0.97                    & 3.2   & 0.82                            & 2             & 0.9                            \\
                                            & total                                & 5.33          & 0.74                    & 6.57  & 0.67                            & \textbf{4.33} & \textbf{0.79}                  \\ 
\hline
\multirow{5}{*}{Bug 7~}                     & shalun                               & -1            & -1.0                    & -1.0  & -1.0                            & -1            & -1.0                           \\
                                            & san                                  & 8             & 0.66                    & 7.2   & 0.7                             & 6             & 0.75                           \\
                                            & gomentum                             & 7             & 0.59                    & 7.4   & 0.57                            & 5             & 0.72                           \\
                                            & cubetown                             & 1             & 0.97                    & 3.4   & 0.81                            & 2             & 0.9                            \\
                                            & total                                & 5.33          & 0.74                    & 6.0   & 0.69                            & \textbf{4.33} & \textbf{0.79}                  \\ 
\hline
\multirow{5}{*}{Bug 8}                      & shalun                               & -1            & -1.0                    & -1.0  & -1.0                            & -1            & -1.0                           \\
                                            & san                                  & 8             & 0.66                    & 11.9  & 0.48                            & 6             & 0.75                           \\
                                            & gomentum                             & 7             & 0.59                    & 7.1   & 0.59                            & 5             & 0.72                           \\
                                            & cubetown                             & 1             & 0.97                    & 3.6   & 0.79                            & 2             & 0.9                            \\
                                            & total                                & 5.33          & 0.74                    & 7.53  & 0.62                            & \textbf{4.33} & \textbf{0.79}                  \\ 
\hline
\multirow{5}{*}{Bug 9}                      & shalun                               & -1            & -1.0                    & -1.0  & -1.0                            & -1            & -1.0                           \\
                                            & san                                  & 8             & 0.66                    & 5.0   & 0.8                             & 6             & 0.75                           \\
                                            & gomentum                             & 7             & 0.59                    & 7.4   & 0.57                            & 3             & 0.84                           \\
                                            & cubetown                             & 1             & 0.97                    & 3.5   & 0.8                             & 2             & 0.9                            \\
                                            & total                                & 5.33          & 0.74                    & 5.3   & 0.72                            & \textbf{3.67} & \textbf{0.83}                  \\ 
\hline
\textbf{Obstacle total}                     & total                                & 5.16          & 0.74                    & 6.61  & 0.63                            & \textbf{4.32} & \textbf{0.77}                  \\
\hline
\end{tabular}
\end{table*}

\begin{table*}
\centering
\begin{tabular}{llllllll} 
\hline
\textbf{Benchmarks (bugs)} & \textbf{Test suite} & \multicolumn{2}{l}{\textbf{Baseline 1}} & \multicolumn{2}{l}{\textbf{Baseline 2}} & \multicolumn{2}{l}{\textbf{Proposed method}}  \\
                           &                     & Top K         & APFD                    & Top K         & APFD                    & Top K         & APFD                          \\ 
\hline
\multirow{5}{*}{Bug 1}     & shalun              & 3             & 0.38                    & 2.0           & 0.63                    & 3             & 0.38                          \\
                           & san                 & 1             & 0.9                     & 1.0           & 0.9                     & 1             & 0.9                           \\
                           & gomentum            & 1             & 0.88                    & 1.0           & 0.88                    & 1             & 0.88                          \\
                           & cubetown            & -1            & -1.0                    & -1.0          & -1.0                    & -1            & -1.0                          \\
                           & total               & 1.67          & 0.72                    & \textbf{1.33} & \textbf{0.8}            & 1.67          & 0.72                          \\ 
\hline
\multirow{5}{*}{Bug 2}     & shalun              & 1             & 0.88                    & 2.0           & 0.63                    & 1             & 0.88                          \\
                           & san                 & 1             & 0.93                    & 2.0           & 0.79                    & 1             & 0.93                          \\
                           & gomentum            & 1             & 0.92                    & 1.0           & 0.92                    & 1             & 0.92                          \\
                           & cubetown            & 2             & 0.7                     & 1.0           & 0.9                     & 3             & 0.5                           \\
                           & total               & \textbf{1.25} & \textbf{0.86}           & 1.5           & 0.81                    & 1.5           & 0.81                          \\ 
\hline
\multirow{5}{*}{Bug 3}     & shalun              & 1             & 0.9                     & 1.0           & 0.9                     & 1             & 0.9                           \\
                           & san                 & 1             & 0.93                    & 2.0           & 0.79                    & 1             & 0.93                          \\
                           & gomentum            & 2             & 0.75                    & 1.0           & 0.92                    & 1             & 0.92                          \\
                           & cubetown            & 2             & 0.75                    & 3.0           & 0.58                    & 1             & 0.92                          \\
                           & total               & 1.5           & 0.83                    & 1.75          & 0.8                     & \textbf{1.0}  & \textbf{0.92}                 \\ 
\hline
\textbf{Signal total}      & total               & 1.45          & 0.81                    & 1.55          & 0.8                     & \textbf{1.36} & \textbf{0.82}                 \\ 
\hline
\multirow{5}{*}{Bug 4}     & shalun              & 1             & 0.75                    & 2.0           & 0.25                    & 2             & 0.25                          \\
                           & san                 & 11            & 0.3                     & 15.0          & 0.03                    & 10            & 0.37                          \\
                           & gomentum            & -1            & -1.0                    & -1.0          & -1.0                    & -1            & -1.0                          \\
                           & cubetown            & 1             & 0.95                    & 6.0           & 0.45                    & 2             & 0.85                          \\
                           & total               & \textbf{4.33} & \textbf{0.67}           & 7.67          & 0.24                    & 4.67          & 0.49                          \\ 
\hline
\multirow{5}{*}{Bug 5}     & shalun              & -1            & -1.0                    & -1.0          & -1.0                    & -1            & -1.0                          \\
                           & san                 & 11            & 0.3                     & 5.0           & 0.7                     & 10            & 0.37                          \\
                           & gomentum            & 3             & 0.69                    & 8.0           & 0.06                    & 4             & 0.56                          \\
                           & cubetown            & 1             & 0.95                    & 3.0           & 0.77                    & 2             & 0.86                          \\
                           & total               & \textbf{5.0}  & \textbf{0.65}           & 5.33          & 0.51                    & 5.33          & 0.6                           \\ 
\hline
\multirow{5}{*}{Bug 6}     & shalun              & -1            & -1.0                    & -1.0          & -1.0                    & -1            & -1.0                          \\
                           & san                 & 11            & 0.3                     & 15.0          & 0.03                    & 10            & 0.37                          \\
                           & gomentum            & 3             & 0.69                    & 4.0           & 0.56                    & 4             & 0.56                          \\
                           & cubetown            & 1             & 0.95                    & 2.0           & 0.85                    & 2             & 0.85                          \\
                           & total               & \textbf{5.0}  & \textbf{0.65}           & 7.0           & 0.48                    & 5.33          & 0.59                          \\ 
\hline
\multirow{5}{*}{Bug 7}     & shalun              & -1            & -1.0                    & -1.0          & -1.0                    & -1            & -1.0                          \\
                           & san                 & 11            & 0.3                     & 5.0           & 0.7                     & 10            & 0.37                          \\
                           & gomentum            & 3             & 0.69                    & 4.0           & 0.56                    & 4             & 0.56                          \\
                           & cubetown            & 1             & 0.95                    & 7.0           & 0.41                    & 2             & 0.86                          \\
                           & total               & \textbf{5.0}  & \textbf{0.65}           & 5.33          & 0.56                    & 5.33          & 0.6                           \\ 
\hline
\multirow{5}{*}{Bug 8}     & shalun              & -1            & -1.0                    & -1.0          & -1.0                    & -1            & -1.0                          \\
                           & san                 & 11            & 0.3                     & 8.0           & 0.5                     & 10            & 0.37                          \\
                           & gomentum            & 3             & 0.69                    & 7.0           & 0.19                    & 4             & 0.56                          \\
                           & cubetown            & 1             & 0.95                    & 2.0           & 0.85                    & 2             & 0.85                          \\
                           & total               & \textbf{5.0}  & \textbf{0.65}           & 5.67          & 0.51                    & 5.33          & 0.59                          \\ 
\hline
\multirow{5}{*}{Bug 9}     & shalun              & -1            & -1.0                    & -1.0          & -1.0                    & -1            & -1.0                          \\
                           & san                 & 9             & 0.39                    & 3.0           & 0.82                    & 9             & 0.39                          \\
                           & gomentum            & 3             & 0.69                    & 4.0           & 0.56                    & 3             & 0.69                          \\
                           & cubetown            & 1             & 0.95                    & 3.0           & 0.77                    & 2             & 0.86                          \\
                           & total               & 4.33          & 0.68                    & \textbf{3.33} & \textbf{0.72}           & 4.67          & 0.65                          \\ 
\hline
\textbf{Obstacle total}    & total               & \textbf{4.78} & \textbf{0.65}           & 5.72          & 0.5                     & 5.11          & 0.59                          \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\begin{tabular}{llllll} 
\hline
\textbf{SUT}                & \textbf{Test suite} & \textbf{TP}  & \textbf{TN}  & \textbf{FP} & \textbf{FN}  \\ 
\hline
\multirow{3}{*}{Signal}     & San                 & 9            & 650          & 0~ ~ ~ ~ ~~ & 1            \\
                            & Gomentum            & 1            & 208          & 0           & 1            \\
                            & Cubetown            & 0            & 210          & 0           & 1            \\ 
\hline
\multirow{3}{*}{Obstacle}   & San                 & 65           & 418          & 0           & 0            \\
                            & Gomentum            & 60           & 308          & 0           & 0            \\
                            & Cubetown            & 55           & 198          & 0           & 0            \\ 
\hline
\multirow{3}{*}{Planning}   & San                 & 300~ ~ ~ ~ ~ & 40           & 0           & 0            \\
                            & Gomentum            & 48           & 112~ ~ ~ ~ ~ & 0           & 0            \\
                            & Cubetown            & 69           & 111          & 0           & 0            \\ 
\hline
\multirow{3}{*}{Prediction} & San                 & 390          & 60           & 0           & 0            \\
                            & Gomentum            & 271          & 269          & 0           & 0            \\
                            & Cubetown            & 429          & 171          & 0           & 0            \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\begin{tabular}{llllllll} 
\hline
\textbf{SUT}                 & \textbf{Test suite} & \textbf{Total bugs} & \textbf{Covered bugs} & \textbf{TP} & \textbf{TN} & \textbf{FP} & \textbf{FN}  \\ 
\hline
\multirow{3}{*}{signal}      & san                 & 5                   & 4                     & 4           & 238         & 30          & 0            \\
                             & gomentum            & 2                   & 1                     & 1           & 178         & 30          & 0            \\
                             & cubetown            & 0                   & 0                     & 0           & 180         & 30          & 0            \\ 
\hline
\multirow{3}{*}{obstacle}    & san                 & 221                 & 186                   & 186         & 180         & 22          & 1            \\
                             & gomentum            & 51                  & 41                    & 41          & 131         & 1           & 22           \\
                             & cubetown            & 181                 & 169                   & 169         & 84          & 0           & 23           \\ 
\hline
\multirow{3}{*}{planning}    & san                 & 20                  & 20                    & 20          & 0           & 0           & 20           \\
                             & gomentum            & 39                  & 38                    & 38          & 91          & 0           & 20           \\
                             & cubetown            & 58                  & 40                    & 40          & 54          & 18          & 2            \\ 
\hline
\multirow{3}{*}{prediction~} & san                 & 390                 & 390                   & 390         & 60          & 0           & 30           \\
                             & gomentum            & 154                 & 94                    & 94          & 206         & 0           & 30           \\
                             & cubetown            & 368                 & 342                   & 342         & 168         & 0           & 30           \\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\begin{tabular}{llllllll} 
\hline
\multirow{2}{*}{\textbf{SUT}} & \multirow{2}{*}{\textbf{Test Suite}} & \multicolumn{2}{l}{\textbf{Baseline 1}} & \multicolumn{2}{l}{\textbf{Baseline 2}} & \multicolumn{2}{l}{\textbf{Proposed method}}  \\
                              &                                      & Top K      & APFD                       & Top K & APFD                            & Top K      & APFD                             \\ 
\hline
\multirow{3}{*}{signal}       & san                                  & 1          & 0.98                       & 2.35  & 0.92                            & \textbf{1} & \textbf{0.98}                    \\
                              & gomentum                             & 3          & 0.64                       & 4.02  & 0.5                             & \textbf{1} & \textbf{0.93}                    \\
                              & cubetown                             & -1         & -1.0                       & -1.0  & -1.0                            & -1         & -1.0                             \\ 
\hline
\multirow{3}{*}{obstacle}     & san                                  & 4          & 0.86                       & 2.76  & 0.91                            & \textbf{1} & \textbf{0.98}                    \\
                              & gomentum                             & 16         & 0.24                       & 8.59  & 0.69                            & \textbf{8} & \textbf{0.9}                     \\
                              & cubetown                             & \textbf{1} & \textbf{0.97}              & 2.0   & 0.92                            & 2          & 0.91                             \\ 
\hline
\multirow{3}{*}{planning}     & san                                  & 1          & 0.97                       & 1     & 0.97                            & \textbf{1} & \textbf{0.97}                    \\
                              & gomentum                             & 7          & 0.26                       & 3.02  & 0.7                             & \textbf{2} & \textbf{0.82}                    \\
                              & cubetown                             & 2          & 0.84                       & 3.33  & 0.72                            & \textbf{1} & \textbf{\textbf{0.94}}           \\
\hline
\end{tabular}
\end{table*}

\begin{table*}
\centering
\begin{tabular}{llllll} 
\hline
\multirow{2}{*}{\textbf{SUT}} & \multirow{2}{*}{\textbf{Test suite}} & \multicolumn{3}{l}{\textbf{Total test time (s)}} & \multirow{2}{*}{\textbf{\textbf{Improvement}}}  \\
                              &                                      & Baseline 1 & Baseline 2 & Proposed method        &                                                 \\ 
\hline
\multirow{3}{*}{signal}       & san                                  & 3.9        & 10.14      & 3.0                    & 70.41\%                                         \\
                              & gomentum                             & 14.42      & 42.94      & 3.0                    & 93.01\%                                         \\
                              & cubetown                             & -1         & -1         & -1                     &                                                 \\ 
\hline
\multirow{3}{*}{obstacle}     & san                                  & 497.54     & 272.96     & 49.61                  & 86.41\%                                         \\
                              & gomentum                             & 1853.71    & 730.76     & 132.06                 & 92.87\%                                         \\
                              & cubetown                             & 105.32     & 279.4      & 129.0                  & 53.83\%                                         \\ 
\hline
\multirow{3}{*}{planning}     & san                                  & 361.06     & 96.0       & 60.0                   & 83.38\%                                         \\
                              & gomentum                             & 1514.16    & 748.49     & 114.0                  & 92.47\%                                         \\
                              & cubetown                             & 437.8      & 586.55     & 60.0                   & 89.77\%                                         \\
\hline
\end{tabular}
\end{table*}
